Towards Physiology-Aware DASH: Bandwidth-Compliant Prioritized Clinical Multimedia Communication in Ambulances

The ultimate objective of medical cyber-physical systems is to enhance the safety and effectiveness of patient care. To ensure safe and effective care during emergency patient transfer from rural areas to center tertiary hospitals, reliable and real-time communication is essential. Unfortunately, real-time monitoring of patients involves transmission of various clinical multimedia data including videos, medical images, and vital signs, which requires use of mobile network with high-fidelity communication bandwidth. However, the wireless networks along the roads in rural areas range from 4G to 2G to low speed satellite links, which poses a significant challenge to transmit critical patient information. In this paper, we present a bandwidth-compliant criticality-aware system for transmission of massive clinical multimedia data adaptive to varying bandwidths during patient transport. Model-based clinical automata are used to determine the criticality of clinical multimedia data. We borrow concepts from DASH, and propose physiology-aware adaptation techniques to transmit more critical clinical data with higher fidelity in response to changes in disease, clinical states, and bandwidth condition. In collaboration with Carle's ambulance service center, we develop a bandwidth profiler, and use it as proof of concept to support our experiments. Our preliminary evaluation results show that our solutions ensure that most critical patient's clinical data are communicated with higher fidelity.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Nowadays with the growing demands of networked applications along with the advancements in networking technologies with support of high bandwidth, while traditional applications such as email, web browsing, music, and video are still popular, there has been a significant rise in the new 3D media such as 3D gaming, 3D videos, 3D virtual environments, and 3D tele-immersive systems. Coming along with Internet 2, 3D tele-immersion technology takes place when individuals at geographically separated sites try to collaborate in a 3D shared virtual environment. Users of an immersive site, or a performer, produce 3D streams by a 3D camera array surrounding their physical space. A 3D model of the performer will then be constructed from the streams and placed on the virtual stage to interact with other users. Thus, the performers can be physically dispersed. The applications are not only used for entertainment, video games and interactive storytelling \cite{ImmersiveApp1}, but also used for other purposes such as biology and tele-medicine for remote health-caring \cite{ImmersiveApp2,ImmersiveApp4}, art \cite{ImmersiveApp3}, as well as military and education \cite{ImmersiveApp1}. Major ongoing research is carried out covering different aspects to deliver 3D immersive experience in real time \cite{3dti1,3dti2,3dti3,3dti4}.

Despite the promising nature of 3D tele-immersion systems, many challenges still remain to make this technology more feasible and available to everyday use. Whi-le we are already witnessing the extreme growth of many live video broadcasting services such as Youtube \cite{youtube}, Livestream \cite{livestream}, and CoolStreaming \cite{coolstreaming}, existing applications of 3D Tele-immersion systems are still restricted with a small number of users. Unfortunately due to the resource limitations such as network bandwidth, one of the major challenges to increase the number of performers and 3D cameras is how to efficiently transmit the bulky 3D stream data to bandwidth-const-rained distributed sites. Unlike the traditional 2D systems such as video conferencing, 3D tele-immersive systems use an array of 3D cameras which in overall leads to a bulky amount of data needed to be transmitted over the networks. Even for a basic setting, the data rate requirement of a single 3D stream may reach up to 100 Mbps and in case of ten 3D cameras in a physical site, the total bandwidth requirement could surpass Gbps level~\cite{yang}. Thus there must be a balance between the requirements of 3D streaming and the architecture of Internet2 backbone. One of the challenges to achieving this balance is to meet the demands for a viewing preference given the limited bandwidth without much negative impact on the user's experience. However our work is motivated by the idea of 3D Tele-immersive amphitheaters with hundred-scale users \cite{shannon} and the bandwidth issues that such rich multimedia system arises, a semantic relation between HVS requirements and multi-ranked stream priorities has not been fully developed for the purpose of the bandwidth management and high performance tele-immersion protocols over Internet2 networks in the previous work. Hence, we propose to utilize this semantic relation in our novel stream adaptation framework, in order to address the concerns and challenges that are neglected by previous research.

In this paper, we study an adaptive HVS-compliant stream management framework for efficient delivery of hundred-scale streams to distributed sites with limited bandwidth budget over networks. Our adaptation framework relies on the concepts of HVS-compliant Field of View (FOV) which exploits the semantics relation of multi-priority 3D streams in the 3D tele-immersive environment, with the main goal of maximizing the total quality of the streamed data to satisfy a bandwidth budget specific to the receiver site. Because of the lack of a fine-grained HVS-compliant prioritized component, many 3D tele-immersion systems extensively experience inefficient resource usage due to the fact that they manage all streams in the same way, with no distinguished importance. Our approach is to selectively choose the proper frame rate, i.e. Frame Per Second (FPS) of each 3D camera given their stream priorities based on FOV of receiver's rendered virtual viewpoint, by limiting the total amount of streamed data to a viewer site while satisfying the bandwidth budget. Our evaluation results show that using our adaptation framework significantly improves the quality per unit of bandwidth consumed to transmit the stream data while it adapts streams according to the users' view preference. In summary, the contributions of this paper include the following: 

\begin{itemize}
\item Feasibility study of a coordinated adaptive stream management system, which enhances the utilization of limited bandwidth issues by incorporating users' view requirements and adaptation.
%\item Definition of HVS-based multi-level stream priorities, which enhances the utilization of limited bandwidth by giving higher priorities to the streams which are semantically more important to the user view. Therefore the framework will provide a view-aware adaptive bandwidth management from users' perspective.
\item Efficient bandwidth management in regards to the hundred-scale prioritized streams, which fine-grains the differentiation of streams and improves the resulting qualities. The computational cost induced by our adaptation mechanism is trivial that makes it suitable for scalability requirements of 3D tele-immersive systems with high number of streams.
\item Development of TELEVIS, a visual simulation tool with a configurable GUI to showcase our HVS-comp-liant adaptations for tele-immersive systems.
\end{itemize}

It should be noted that this paper is an extended study of our previous conference version \cite{mmve15}, which is extended by 70\% relative to the prior study. The new contribution includes a) development of TELEVIS visual simulation tool, which models the interaction of participants using facing and clustering algorithms, b) comparison of the relative execution time overhead of our proposed algorithm against BLMCK algorithm \cite{blmck}, tested for large number of streams, and c) the discussion of runtime overhead for the main proposed heuristic in Section 3.4. In addition, our extended paper discusses more details, including an extended introduction and more thorough discussion of related work.

The paper is organized as follows: in Section \ref{sec:background}, we cover a wide area of related work, and we discuss how our system is related to them. Section \ref{sec:methodology} explains our methodology for adaptive stream management system, including the problem definition and the stream prioritization. Our evaluation results are presented in Section \ref{sec:evaluation}, while in Section \ref{sec:conclusion} we conclude the paper and briefly discuss possible improvements for future work.


==> scenario.tex <==
\section{Prioritization in Emergency Acute Disease Care}
\label{sec:scenario}
In this section we elaborate on emergency care for acute diseases as real-world use cases, and illustrate how various clinical data priorities might have different criticality levels within the context of a specific episode of acute disease patient care transport. To clarify the concepts, we describe acute stroke as the leading example of emergency acute disease care in details, followed by a scenario of car accident emergency care and transport.
\subsection{Stroke}
Stroke is the third leading cause of death and the first leading cause of disability in the United States~\cite{stroke-stats}. In addition, stroke patients are often elderly (in fact, 65\% to 72\% stroke patients are over age 65~\cite{elderly-stroke-rate}) who may have the highest communication priority. Furthermore, some effective stroke treatment medications have strict implementation guidelines; these may begin at the remote facility and continue through ambulance transport to the receiving regional hospital center. Overall, different factors and features may take priority when considering communication and limiting bandwidth availability.

Figure \ref{fig:example-tpa} shows the envisioned workflow for a stroke patient care from rural facility to a regional hospital center. Consider a 70 year old male patient who arrives at a rural hospital. It is determined clinically that the patient has the sudden onset of stroke. Computerized Tomography (CT) scan is completed at the remote rural medical facility; the CT images are sent to the stroke team at the center hospital for further immediate interpretation. At this time, CT scan is critical and the transmission of data associated with the images has the highest communication priority. The CT can be completed in the rural hospital depending on the radiologic device availability, or inside a mobile stroke unit such as a CT scan-equipped ambulance \cite{mobilestroke}. Patient's primary vital signs, measurements and indexes, including blood pressure, heart rate, and blood oxygenation (SpO$_2$) are collected immediately as necessary. Patient's biometric information can also be retrieved, sometimes using the camera mounted on a mobile device, and sent as lower priority. With the assistance of healthcare providers at the regional center hospital via real-time monitoring (we collaborate with Carle Foundation Hospital as the center hospital \cite{carle} in Champaign county), the physicians and nurses in the rural facility determine the patient's state and the treatment plan.

If it is determined that the patient has a hemorrhagic stroke\footnote{Hemorrhagic stroke occurs when a blood vessel bursts inside the brain, which damages the nearby brain tissue.} (and not an ischemic stroke caused by blood clots), the patient will be sent immediately to the regional center hospital as specialist physicians and specialized treatments (interventional neuroradiology as example) may be required. In the ambulance, supportive measures begin and the center hospital is notified and calls in the team of specialized care for the patient. For this patient, time of transport is most critical. Clinical concerns in the ambulance focus on blood oxygenation and respiratory function. Laboratory values and ordinary vital signs assume less importance in comparison so long as they remain mostly within normal ranges. Thus, somewhat elevated blood pressure may be tolerated and an elevated blood glucose of 350 may observed until arrival at the regional hospital center. The patient is monitored closely however for change in neurological (clinical) status. %If possible, the coordination of results from common blood clotting laboratory studies are rapidly facilitated, which may include INR, PTT, and TEG examination.

If the patient has ischemic stroke\footnote{Ischemic stroke occurs when a blood clot blocks an artery headed to the brain.} (much more common than a hemorrhagic stroke) and is in a stable state, in consultation with the regional center a standard treatment may be to begin an infusion of a clot dissolving medication such as tissue plasminogen activator (tPA). The patient will be sent to the center hospital with the infusion of tPA flowing intravenously. Unfortunately, many patients with ischemic stroke are in an unstable state, that is, vital signs are seriously out of range and must be treated actively. In such a modeled scenario case, the patient with an ischemic stroke but unstable vital signs is placed on the ambulance accompanied with a stroke bag carrying needed equipment, blood products and treatments to manage care during transport and reduce the patient's risk of further deterioration.

tPA is a common intravenous treatment to dissolve a blood clot which occludes a vital artery supplying blood to the brain. A significant risk of the use of tPA to dissolve an occluding blood clot that has caused a stroke is the complication of bleeding as tPA alters the body's blood clotting mechanism. As many elderly patients already take chronic medications to reduce the possibility of blood clots anyplace in the body, it can be important to know the precise nature of the body's effective blood clotting ability. To study such patient with stroke and who may already be taking anti-coagulation medication, the TEG\footnote{Thromboelastography (TEG) is a method of testing the efficiency of blood coagulation, which helps with timing tPA and clot dissolving therapy.} is performed at the remote facility or in the ambulance and the results of this blood examination is sent to the receiving hospital facility for consideration. Transmission of data associated with TEG measurements has high priority to avoid complication of brain hemorrhage. Assuming a TEG examination can be performed at the distant rural facility or the blood can be drawn and studied in the ambulance in a mobile TEG lab unit, the expert consults at the central receiving hospital may use the TEG to address the infusion of tPA itself or plan on the approach to further anticoagulation therapy in the face of complicating features. In addition to TEG measurements, patient's neurological symptoms such as speech difficulty, facial droop, weakness in hands as well as vital signs including the blood pressure, heart rate, SpO$_2$, blood glucose level, and blood coagulation index will also be monitored in real-time in the center hospital, at the rural hospital and the ambulance during transport. In these situations, transmission of vital signs has higher priority compared to the clinical data associated with patient's voice for speech difficulty, and audio-visuals taken to determine levels of facial droopiness and hand weakness. If any of the vital signs are out of range, the stroke team in the center hospital will work with the ambulance staff to manage treatment orders and the additional requirements that arise from a changing patient state. Let's take blood pressure as an example of remote monitoring. When the patient's blood pressure exceeds the safe threshold 180, the stroke team of the center hospital may suggest injecting the IV infusion of a medication such as nicardipine or nitroprusside to control the blood pressure. If the nicardipine or nitroprusside infusion does not control the elevated blood pressure, the physician of the center hospital may change treatment accordingly. Here, a ``blood glucose level'' that cannot be controlled within acceptable clinical range is an important measurement value at this situation which requires close coordination among the ambulance staff and the expert physicians at the central facility. Clearly, to minimize the patient's risks during transport, real-time supervision and monitoring of the stroke team in the ambulance is crucial, because the majority of stroke patients are elderly with various chronic diseases characterized by many complicating features. Even if such elderly patients are initially in a stable state, they may become unstable with various complications under the stress of stroke. Overall, the variations of both the required clinical data and their priorities at each patient and disease state is an important motivation in driving this research. Thus in the example of a reasonably stable patient with ischemic stroke during transport, the most critical information to dominate communicate should relate to blood pressure control, and change in neurologic clinical status while the tPA is infusing. Of less criticality are more ordinary clinical data such as blood glucose, which can be addressed on arrival.
\begin{figure*}[!t]
\centering
\includegraphics[width=1\textwidth, trim = 50 60 30 60, clip = true]{scheme.pdf}
\vspace{-1cm}
\caption{An example scheme of proposed adaptation approach.}
\vspace{-.5cm}
\label{scheme}
\end{figure*}
\subsection{Car Accident}
Similar to the context of a stroke patient, let's consider an emergency situation where a car accident has happened, and the patient is picked up by an ambulance. There is a head injury and obvious wound of the scalp, and it is difficult to control bleeding. In this case, if the vital signs are maintained and laboratory data are within threshold limits according to the patient status models, and assuming maximum bandwidth is available, bandwidth is allocated per protocol. But lets consider the blood pressure level is 190/- and the patient is elderly and has a history of high blood pressure which is common. The disease models indicate that hematocrit is 30 (low) and the bleeding continues (these are real situations in car accident emergency). Travel time to the hospital (definitive help) is more than an hour, and patient's glucose level is 350. Here, the glucose measure might be ignored as in bleeding measurement of hematocrit is primary and has higher priority than treatment of high blood pressure and measurement of glucose levels. In this case, the blood pressure of 190/- is not treated even though it is high and known to be associated with worsening head and brain injury. If the ambulance staff treat the patient's blood pressure to a more desirable level (e.g 150 in this case), there is a risk of worsening the blood pressure to a level below 100/- due to the patient's continuous bleeding (the blood pressure continues to go down on its own as bleeding continues and worsens the situation). Here, controlling the bleeding scalp has higher priority compared to the brain injury, which is the current best practice in how this situation is handled in a safe manner. Therefore, if bandwidth is limited, much less importance is devoted to the data associated with the audio-visual streams, periodic neurological examination data of head injury, and other laboratory data. Once maximum bandwidth returns, all of the clinical data transmission returns to standard protocol.​
 
Now let's consider a similar situation, but a different patient. A car accident has occurred, and the patient has brain injury with blood pressure level 190/- and hematocrit level of 30 (normal), however, with no scalp injury. The patient is seen to be deteriorating neurologically, and there is no scalp wound or suspicion of any injury that would cause bleeding. The blood glucose level is measured as 350. Here, as the first step, the blood pressure should be lowered immediately. Next issue to be considered is to give insulin to lower the glucose level, while the last issue would be to watch the hematocrit measures and possibly repeat this process for reassurance. Therefore, at the first state, blood pressure measurements has higher priority compared to other clinical data including glucose, hematocrit measurements, and other audio visual clinical data. The assumption here is that in the absence of an injury that might cause bleeding, the hematocrit of 30 is a chronic condition and not related to the injury. In this situation, this would be confirmed as the third priority. That said, hematocrit measurements are repeatedly done to be certain it does not change, and then monitoring the blood pressure so that it does not fall too far when medications are given to lower the dangerous 190/- level as well watching the heart rate levels are least priority. Here the heart rate should be 90-110 as a normal response to injury. If it is higher or inconsistent with the situation, there is a possibility of bleeding. Overall, one a patient state as described above, transmission of blood pressure has highest bandwidth priority, while measurements of insulin and the hematocrit levels have secondary bandwidth priority which are actually for reassurance and re-evaluating the patient' clinical situation.
